Detection of very-high-energy {\gamma}-ray emission from the colliding wind binary {\eta} Car with H.E.S.S

Aims. Colliding wind binary systems have long been suspected to be high-energy (HE; 100 MeV < E < 100 GeV) {\gamma}-ray emitters. {\eta} Car is the most prominent member of this object class and is confirmed to emit phase-locked HE {\gamma} rays from hundreds of MeV to ~100 GeV energies. This work aims to search for and characterise the very-high-energy (VHE; E >100 GeV) {\gamma}-ray emission from {\eta} Car around the last periastron passage in 2014 with the ground-based High Energy Stereoscopic System (H.E.S.S.). Methods. The region around {\eta} Car was observed with H.E.S.S. between orbital phase p = 0.78 - 1.10, with a closer sampling at p {\approx} 0.95 and p {\approx} 1.10 (assuming a period of 2023 days). Optimised hardware settings as well as adjustments to the data reduction, reconstruction, and signal selection were needed to suppress and take into account the strong, extended, and inhomogeneous night sky background (NSB) in the {\eta} Car field of view. Tailored run-wise Monte-Carlo simulations (RWS) were required to accurately treat the additional noise from NSB photons in the instrument response functions. Results. H.E.S.S. detected VHE {\gamma}-ray emission from the direction of {\eta} Car shortly before and after the minimum in the X-ray light-curve close to periastron. Using the point spread function provided by RWS, the reconstructed signal is point-like and the spectrum is best described by a power law. The overall flux and spectral index in VHE {\gamma} rays agree within statistical and systematic errors before and after periastron. The {\gamma}-ray spectrum extends up to at least ~400 GeV. This implies a maximum magnetic field in a leptonic scenario in the emission region of 0.5 Gauss. No indication for phase-locked flux variations is detected in the H.E.S.S. data.

==> HESS_journal_v3_proof.tex <==
\section{H.E.S.S. data analysis}
\label{sec:analysis}

\subsection{H.E.S.S. data}
\label{sec:nsb_trigger}
The \hess\ experiment is an array of five Imaging
Atmospheric Cherenkov Telescopes (IACTs) located in Namibia. It
is the only IACT system integrating different telescope types
into one array and is sensitive to \g-ray emission from Galactic and
extragalactic sources in the energy range from
$\sim$$30$\,GeV to tens of TeV. The four H.E.S.S.-I telescopes are
equipped with mirrors of 12\,m diameter and have a Davies-Cotton
  mirror geometry. The larger CT5 telescope has a parabolic mirror diameter of 28\,m,
which makes it the largest IACT worldwide. The field of view (FoV) of
the H.E.S.S.-I telescopes is 5$\,^{\circ}$ in diameter, whereas CT5 has a FoV of
$\sim$3.2$\,^{\circ}$ \citep{Bolmont2014}. The addition of CT5 to the
array significantly lowered the energy threshold, allowing for a
broader overlap in energy in the transition region between \hess\ and space-based
instruments like \fermi.

The main challenge in the analysis of \g-ray data from the direction
of \EC\ is the large number of UV photons originating from the Carina
Nebula that cause a significant increase in NSB, causing fake
triggers of the telescope and increasing noise levels in the image
pixels. For instance, the NSB rate in the Galactic plane is
typically around 100\,MHz per pixel in the image. This translates to a mean
number of NSB photons of 1.6 photo-electrons (p.e.) per
pixel. The NSB in the direction of \EC\ is up to ten times higher than
the Galactic average and varies greatly across the FoV. To distinguish
real Cherenkov showers from
NSB-induced events, at least three neighbouring pixels with
$>4.0$\,p.e. above the average NSB are required to trigger the CT5 camera. The
resulting telescope trigger rate is 1.5 kHz, mostly from genuine air
showers. In the case of \EC\ this threshold was applied for
data set I (DS-I; see Tab.~\ref{tab:data}), while CT5 camera HV
adjustments required to increase the pixel trigger thresholds to
4.5\,p.e. for data set~II (DS-II).

\begin{table}
  \centering
  \caption{Properties of the data sets used in this work to
    calculate the spectral points and the light-curve shown in
    Fig.~\ref{fig:Spec} and \ref{fig:LC}, respectively. The time interval
    of the \hess\ observations, the total live time corresponding to
    the individual data sets, along with the covered orbital phase are summarised.}
  \begin{tabular}{@{}ccccc}
    \hline
    Data Set & Observation Time & Phase & live time \\
    (DS) & Modified Julian Date (MJD) & & (hours) \\ \hline
    I & $56439 - 56444$ & 0.78 & 0.9 \\
      & $56666 - 56667$ & 0.89 & 0.8 \\
      & $56741 - 56751$ & 0.93 & 9.4 \\
      & $56775 - 56778$ & 0.95 & 0.9 \\
      & $56797 - 56799$ & 0.96 & 1.8 \\ \hline
   II & $56803 - 56807$ & 0.96 & 3.3 \\
      & $57066 - 57074$ & 1.09 & 8.6 \\
      & $57077 - 57079$ & 1.10 & 4.0 \\ \hline
 all  & $56439 - 57079$ & $0.78 - 1.10$ & 29.7 \\ \hline
  \end{tabular}
  \label{tab:data}
\end{table}

Observations in the direction of \EC\ were
mainly performed in the first six months of 2014 and 2015 (with the
exception of one observation, which was conducted in May/June
2013). The properties of the individual data sets are summarised
in Tab.~\ref{tab:data}. \EC\ was observed with only CT5 for DS-II,
which limits the analysis to monoscopic
data. The data quality of DS-I and DS-II has been checked with
standard tools. To adjust to the high NSB level and the extra pixels
turned off to protect the Cherenkov camera, the requirement on the
maximum relative fraction of deactivated pixels per observation in CT5 has
been relaxed from 5\% to 10\% \citep[cf][]{2017AGNHessII}.

\subsection{H.E.S.S. data analysis}
\label{sec:hess_analysis}
The \EC\ data have been analysed using two software packages with
independent shower simulation, calibration, reconstruction and
\g/hadron separation to cross check the results. Results presented in
this paper were produced with the \textit{model analysis}
\citep{2009DeNaurois}, which is based on a semi-analytical model for
the electromagnetic shower development in the atmosphere to infer the
properties of the primary particle. All results have been successfully
cross-checked in the {\textit{HAP} framework, which employs a
neural-network based shower reconstruction and \g/hadron separation
\citep{Murach2015}.

\begin{figure*}[ht!]
  \begin{minipage}{0.595\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/EC_NSB_PostMono_SignCont3d5_4d75_6.png}
\end{minipage}
\begin{minipage}{0.395\textwidth}
  \includegraphics[width=0.9\textwidth]{figures/EC_GammaAccMap_all.pdf}
  \includegraphics[width=\textwidth]{figures/EC_acceptance_asymmetry_profiles.pdf}
\end{minipage}
\caption{\label{fig:NSB} {\it Left:} Smoothed NSB rate per camera pixel in MHz
  for CT5 overlaid with contours for 3.5, 4.75 and 6 $\sigma$ of the mono
  analysis of DS-I and DS-II. Turned-off pixels are
    treated as 0\,MHz, hence the map illustrates the average NSB
    operating pixels are exposed to. The optical position of \EC\ is denoted
  with a small star. {\it Right:} Zoom into the 2D \g-ray acceptance 
    map (top) and the relative asymmetry in RA and Dec (bottom).}
\end{figure*}

The NSB in the \EC\ FoV as shown in Fig.~\ref{fig:NSB}
poses serious challenges for the instrument and the \g-ray
data analysis. As described in \citet{Aharonian2004}, the NSB rate can
be inferred for every camera pixel without Cherenkov light signal
based on the pedestal width. Additional checks and systematic tests have been
performed to study its influence on the calibration, shower
reconstruction, and \g/hadron separation. These tests are described in
more detail in the following.

The Carina Nebula is extended over a $\gtrsim0.3^\circ$ region, which is comparable to the Cherenkov image size of low-energy
showers (cf. Fig.~\ref{fig:NSB}). Noise triggers could hence locally
mimic low-energy extensive air showers. The goal
was to reduce the impact of noise-induced triggers as early as
possible in the analysis chain. Therefore, the main and cross-check analysis
apply an image cleaning procedure to provide the seed for the
likelihood fit \citep[see below][]{2009DeNaurois}, and to reject noise pixels in
the image analysis \citet{Aharonian2004}, respectively. The nominal
dual-threshold cleaning of 4\,p.e. for a pixel and 7\,p.e. for a
neighbour pixel (i.e. (4,7) cleaning) has been increased to a (6,12)
cleaning.

As a next step, a pixel-wise log-likelihood comparison between the
predicted Cherenkov shower images, taking into account the NSB and
electronic noise, and the images recorded by the telescopes is
performed. This fit provides an estimate for the energy and direction
of the incident particle \citep{2009DeNaurois, Holler2015}. The
semi-analytical model also provides a \textit{goodness of fit}
parameter and the reconstructed primary interaction depth that are
used to discriminate \g-ray events from hadronic background. In
addition, the estimated error on the reconstructed direction of
each event is required to be smaller than 0.3$^{\circ}$.

To control the NSB, a \textit{uniform NSB goodness} variable was
defined, which characterises the likelihood of accidentally
triggering on fluctuations caused by NSB. In contrast to the
\textit{NSB goodness} variable as introduced in \citet{2017AGNHessII},
the \textit{uniform NSB goodness} parameter assures a flat acceptance
to background-like events, at the cost of an inhomogeneous
acceptance to \g-ray like events. Although the number of accidental
NSB camera triggers are reduced to a manageable level, NSB 
photons are still recorded, when real Cherenkov-induced events
trigger the array and are recorded. The reduction in NSB-only
events by applying these cuts and the response
of the instrument is demonstrated in Fig.~\ref{fig:NSB},
right. Here, the acceptance to \g-ray like background events is
  shown for DS-I and DS-II. The asymmetry in RA and Dec expressed as
  $(x - (-x)) / (x + (-x))$ across the \EC\ FoV is stable at the 5\%$
  - $10\% level. This shows that the
influence of NSB on the background extraction is generally under
control. For the generation of sky images, the \textit{ring
  background} technique is used, while for the spectrum
determination the \textit{reflected background} method is used
\citep{Berge2007}.

\subsubsection{VHE \g-ray detection}
The analysis of data acquired in \hess\ observations towards \EC\
before 2011, and published in \citet{Abramowski2012}, yielded an energy
threshold of 470$\,$GeV. For the CT5 mono analysis presented in
this work, and the modifications made as described above, the
energy threshold is 190\,GeV and 220\,GeV for DS-I and DS-II,
respectively. Figure~\ref{fig:MonoSign} shows the VHE \g-ray
significance map of the sky in the direction of \EC\ for all monoscopic events from 
both data sets that pass \g/hadron separation cuts as described in the
previous section. Significant VHE \g-ray emission is also seen in DS-I
and DS-II separately. In the signal region, centred at the
position of \EC, a \g-ray excess of ($526\pm 62$) events above
background at a significance level of 8.9\,$\sigma$ is found in DS-I. In
DS-II, the \g-ray excess is $541\pm 56$ at a statistical significance
of 10.3\,$\sigma$. The emission seen in DS-I with the mono analysis is
also confirmed, but at a lower significance of 7.2\,$\sigma$, with the
CT1-5 stereo analysis. This can partly be explained by the increased
energy threshold of the stereo analysis. Also, the cross-check analysis
confirms the significant detections in both data sets. 

The maximum of the \g-ray emission shown in Fig.~\ref{fig:MonoSign}
stems from the direction of \EC\ and not from the region of highest
NSB. Outside of the signal region, the distribution of sky map
significance is roughly consistent with the expected normal
distribution, showing a width of 1.04 and 1.08 in DS-I and DS-II,
respectively. The maximum of the NSB, as shown in Fig.~\ref{fig:NSB},
does however coincide with some residual \g-ray like emission south of
\EC. The origin of this feature and its implication for the \EC\
measurement are discussed in the following.

\begin{figure}[ht]
\centering
\includegraphics[width=0.495\textwidth]{figures/EC_ModelMono_All_Sign_psf_4FGL.png}
\caption{\label{fig:MonoSign} Significance map as obtained
  in the CT5 mono analysis, for the combined DS-I ($0.78 < p < 0.96$)
  and DS-II ($1.09<p<1.10$) using an oversampling radius of
  0.1$^{\circ}$. The position of \EC\ is denoted with a black
  star and the long-dashed ellipse refers to the uncertainty in
  the positional fit as described in the main text. The positions of
  the nearby \fermi\ sources 4FGL~J1048.5$-$5923 and
  4FGL~J1046.7$-$6010 are shown with blue crosses
  \citep{Fermi4FGL}. The inlay shows the point spread function (PSF)
  as obtained using run-wise simulations (RWS) in colour, while the overlaid dotted circle
  indicates the PSF using classical simulations.}
\end{figure}

As a first step, we attempt to determine the morphology of the \g-ray
emission based on Fig.~\ref{fig:MonoSign} and the \g-ray maps of the
individual data sets. In ground-based \g-ray astronomy, instrument
response functions (IRFs) are typically produced using Monte-Carlo
(MC) simulations at fixed phase space points and assuming an ideal
detector (no turned-off pixels, uniform NSB, no telescope
tracking). The point spread function (PSF), however, is influenced by
the high NSB level: NSB photons can enter the reconstruction, which
leads to noisier shower images and hence an increased PSF. For complex
FoVs and measurements at the systematic limit, this approach is not
accurate enough anymore. It has been shown that a realistic
description of the observing conditions and instrument properties
under which \g-ray data has been taken is crucial when deriving the
PSF of \hess\ in measuring the extension of the Crab Nebula at TeV
energies \citep{AbdallaCrab2019}. With its challenging observing
conditions, the analysis presented here is another prime example for
the utility of this approach. In the following, we employ the usage of
run-wise simulations (RWS) to derive the PSF of DS-I and
DS-II. Although this more realistic description represents a
significant improvement over the classical IRFs, we note that due
to computational limitations, only the \g-ray signal is simulated
and not the cosmic-ray background, whose uniformity across the FoV
will be impacted by the increased and inhomogeneous NSB. A
non-uniformity in cosmic-ray background will impact the precision of
the background subtraction required to extract the \g-ray signal.

Positional fits of the \g-ray emission of DS-I and DS-II have
been performed using RWS assuming different underlying spectral indices
of the emission. Assuming a spectral index of $\Gamma=3.7$, consistent with
the spectral result discussed below, the morphology fit on DS-II (the
data set, which shows the lowest instrumental systematics) results in
a morphology consistent with being point-like and a best-fit
position of RA=\HMS{10}{44}{35}$\pm 6.6^{\mathrm{s}}$ and
Dec=\DMS{-59}{39}{56.6}$\pm 0.8'$ (J2000), $3.8'$ away from the optical
\EC\ position. To estimate the systematic uncertainty of the derived
best-fit position of data taken under different observing and
instrument conditions, morphology fits to DS-I and DS-II in the RWS
framework, and with classical IRFs in both the main and cross-check
analysis were performed. The derived best-fit position depends, for
instance, on the assumed underlying power-law spectral index, which
was varied between $\Gamma=3.0$ and $\Gamma=4.0$. The systematic error
on the position is estimated following this description as
$\Delta$RA=$\pm 1.5^{\mathrm{m}}$ and $\Delta$Dec=$\pm
4.8'$. Within the statistical and systematical error, the
derived best-fit position is consistent with the optical position of
\EC. The consistent treatment of the NSB by using RWS
is necessary to reconstruct a source that is compatible with being
point-like at the \EC\ position. 

Another complication in the determination of the source morphology is
the assumption of a single component as origin of the \g\
rays. Figure~\ref{fig:MonoSign} suggests that a weaker emission component
south of \EC\ exists and possibly biases the 2D morphology
fit. A dedicated analysis was performed towards this emission component at
RA=\HMS{10}{44}{22.8} and Dec=\DMS{-59}{57}{51.8} (J2000), which results
in a hotspot at 6.5$\,\sigma$ level in DS-II -- dubbed
HOTS~J1044$-$5957. At this significance level, and given the fact that the emission is located in
the region with the highest NSB in the FoV, we do not claim a new
source, but we note that not fully understood systematics could explain at
least parts of this emission. The contribution of HOTS~J1044$-$5957 to the
\EC\ emission is estimated to $\sim$15\%, based on a Gaussian fit
to the 1D spatial profile along the axis connecting \EC\ and
HOTS~J1044$-$5957. 

We emphasise that the hotspot is not detected in the cross-check
analysis, neither in DS-I nor in DS-II. This further supports that
the hotspot seen in the main analysis may be caused by a systematic
effect, likely the response of the classifying parameters to the
NSB. Also, at lower \g-ray energies, no counterpart is reported in
the \fermi\ 4FGL catalogue \citep{Fermi4FGL}. The spectral
properties of \EC\, as presented in the next section, are well
compatible within errors in the main and cross-check analysis,
implying a robust spectral measurement within uncertainties. To
conclude, all tests confirm the integrity of the signal, and given the
good positional coincidence, we assume in the following that it is
connected to the CWB system. The potential impact of the systematics
discussed above will be addressed as systematic error on the inferred
spectral measurement, as described in the next section.

\subsubsection{VHE \g-ray spectrum and light-curve}

\begin{figure}
\centering
\includegraphics[width=0.495\textwidth]{figures/EC_Spectrum_syst_v2.pdf}
\caption{\label{fig:Spec}Spectral energy distribution of \EC\ for DS-I (black)
  and DS-II (red). H.E.S.S. points show 1$\sigma$ statistical
  errors. The shaded regions indicate the combined statistical and systematic
  errors (as given in the main text and Tab.~\ref{tab:syst}). \fermi\ 
  spectra from \citet{Reitberger2015} for the full orbit (grey) and
  for the last periastron passage from \citet{Balbo2017} (blue) are
  also shown.}
\end{figure}

In the following, the intrinsic \g-ray spectrum is reconstructed
and the \g-ray signal is checked for variability and phase-locked
  flux variations as seen at other wavelengths. To enclose the entire
emission seen from \EC, the \textit{reflected background} method
\citep{Berge2007} was used with an on-source region radius of
0.2$^\circ$, and the forward-folding technique by \citet{Piron2001}
is applied to extract spectral parameters. RWS are currently
limited to the simulation of point sources of \g\ rays. For the
spectrum reconstruction one typically assumes that the response to
\g-ray like background events is identical in the signal and
background control regions. The number of turned-off pixels is much
higher towards \EC\ than in the surroundings. Hence, the response to
\g-ray like background events will also be different. For these
reasons, we use in the following classical IRFs.

Figure~\ref{fig:Spec} shows the spectra for DS-I and DS-II for the
mono analyses. The best-fit spectral index for DS-I is
$\Gamma_{\mathrm{DS-I}} = 3.94\pm 0.35_{\mathrm{stat}}$ above an energy
threshold of 190\,GeV. The flux normalisation at the decorrelation
energy \footnote{The decorrelation energy $E_0$ is defined as $E_0 =
  \exp{\frac{cov(F_0,\Gamma)}{F_0\Delta\Gamma^2}}\,\mathrm{GeV}$ \citep{Abdo2009},
  where $cov$ is the covariance error matrix.} of
$E_{\mathrm{0,DS-I}} = 290$\,GeV is $F_{0,\mathrm{DS-I}} = (5.1\pm 0.5_{\mathrm{stat}}
)\times
10^{-11}$\,ph\,cm$^{-2}$\,s$^{-1}$\,TeV$^{-1}$. The \g-ray
spectrum for DS-II above an energy threshold of 220$\,$GeV is best
described by a power-law with index of $\Gamma_{\mathrm{DS-II}} =
3.49\pm 0.23_{\mathrm{stat}}$ and normalisation $F_{0,\mathrm{DS-II}} = (3.2\pm 0.3_{\mathrm{stat}}) \times
10^{-11}$\,ph\,cm$^{-2}$\,s$^{-1}$\,TeV$^{-1}$ at a decorrelation
energy of $E_{0,\mathrm{DS-II}} = 360$\,GeV. The DS-II spectrum is
within statistical errors consistent with the DS-I spectrum (see Tab.~\ref{tab:spec}).

\begin{table*}
  \centering
  \caption{Spectral statistics for the two
      analyses. Uncertainties are statistical. $\mathrm{E_{th}}$
    denotes the threshold energy, $\mathrm{E_{0}}$ the decorrelation
    energy, and $\Phi_0$ the flux at the decorrelation energy.}
  \begin{tabular}{@{}ccccccc}
    \hline
    DS &$\mathrm{E_{th}}$ & $\Gamma$ & $\mathrm{E_{0}}$ & $\Phi_0$ & $\Phi(>0.2)$\,TeV\\ 
       & [TeV] & & [TeV]
       & $[\mathrm{cm}^{-2}\,\mathrm{s}^{-1}\,\mathrm{TeV}^{-1}]$
       & $[\mathrm{cm}^{-2}\,\mathrm{s}^{-1}]$\\ \hline
    I & 0.19 & 3.94 $\pm$ 0.35& 0.29 & (5.1 $\pm$ 0.5) $\cdot10^{-11}$ & (1.6 $\pm$ 0.2)  $10^{-11}$\\
    II & 0.22 & 3.49 $\pm$ 0.23 & 0.36 & (3.2 $\pm$ 0.3) $\cdot10^{-11}$ & (2.0 $\pm$ 0.2)  $10^{-11}$\\
  \end{tabular}
  \label{tab:spec}
\end{table*}

Several sources of uncertainty influence these spectral measurements. 
They range from MC simulations of the air-shower and the instrument,
the calibration, and data quality selection, to the high-level
reconstruction, \g-ray selection, and background
estimation. Table~\ref{tab:syst} lists all contributions to the flux
normalisation and spectral index uncertainty and is based on
\citet{2017AGNHessII}. The
systematic error from switched-off pixels has been increased from
the nominal 5\% to 10\% to reflect the conditions in this
analysis. Errors on the spectral index and normalisation from uncertainties
in the reconstruction and selection cuts are based on differences
between the main and cross-check analysis. The downward systematic
errors resulting from uncertainties in the background subtraction,
as discussed at the end of the previous section, were estimated from
the reconstructed integral flux of HOTS~J1044$-$5957 in DS-II. 
Furthermore, we note that the reconstructed spectrum of the lead
analysis may be prone to a shift of the energy scale of 20\% towards lower
energies. Even with this potential bias, the shifted spectral points
would still be captured by the systematic error budget estimate
presented in Tab.~\ref{tab:syst} and Fig~\ref{fig:Spec}. We
emphasise that the re-binned spectral points are shown only to guide
the readers eye and cannot easily be combined with \fermi\ data
points in a multiwavelength spectral fit.

\begin{table*}[ht]
  \caption{Estimated contributions to the systematic uncertainties in
    the spectral measurements for the mono analyses presented in this
    work follow the description in \citet{2017AGNHessII} and we assume
    similar systematics as for the PG~1553+113 source, which has a similarly
    steep spectral index as \EC. Values quoted are for upward /
    downward or symmetric errors. See text for more details on
    the differences. The energy scale uncertainty in this analysis is
    estimated to be larger than for PG~1553+113.}
\centering
\begin{tabular}{c c c c c c c}
\hline
Source of Uncertainty & Energy Scale & Flux & Index & Flux & Index\\
 & & DS-I & DS-I & DS-II  & DS-II \\
\hline
MC shower interactions			& & 1\%	&  & 1\%  & \\
MC atmosphere simulation		& 7\% & & & & \\
\hline
Instrument simulation / calibration	& 10\% & 10\% & & 10\% & \\
Broken pixels				& & 10\% & & 10\% & \\
Live Time				& & $<5\%$ & & $<5\%$ & \\
\hline
Reconstruction and selection cuts	& 15\%	& 15\%
                                            & 0.96 & 15\% & 0.34 \\
Background subtraction			& & 10\% / 55\% & 0.46 & 10\%
                                                                 / 55\% & 0.46 \\
\hline
Total					& 19\%	& 24\% / 60\%
                                            & 1.06  & 24\% / 60\% & 0.57 \\
\hline
\end{tabular}
\label{tab:syst}
\end{table*}

Figure~\ref{fig:LC} shows the \g-ray light-curve of \hess\ for the data
described in Tab.~\ref{tab:data}. All flux points with a
statistical significance of more than 2$\sigma$ are displayed as
points, whereas upper limits at 95\% confidence level are shown for
non-significant flux measurements. The \hess\ light-curve is
within uncertainties consistent with no variability\footnote{The
    probability for a constant flux in nightly and monthly bins,
    including fits to the deep-exposure data sets at p=0.95 and
    p=1.09, is at the 0.5\% level. When including systematic errors,
    this probability increases and the search for variability is
    non-significant at the $1.5 - 2.0$ $\sigma$ level.} This is in
agreement with the \fermi\ high-energy light-curve that is, however,
rather limited in statistics and can only probe the \g-ray emission on
much longer timescales. In the following, we will put the
\hess\ results in the multiwavelength context and discuss what they
imply for particle acceleration and \g-ray emission processes in this
unique object. 

\begin{figure}
\centering
\includegraphics[width=0.475\textwidth]{figures/HESS_Swift_LC_v2.png}
\caption{\label{fig:LC} Phase-binned \hess\ flux above 190$\,$GeV as
  red points. The phase errors in the \hess\ light-curve
  points refer to the re-grouped data given in
  Tab.~\ref{tab:data}. \fermi\ \g-ray flux points from \citet{Balbo2017} and
  Swift X-ray data from \citet{Corcoran2017} are shown as green triangles
  and as black line, respectively. Flux errors are all 1$\sigma$
  while upper limits are 95\% confidence level. The X-ray data has
  been scaled to arbitrary units for better comparison to the \g-ray
  data.}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "EtaCar_HESS2_rev1"
%%% End:

